Production of associated $\Upsilon$ and open charm hadrons in $pp$ collisions at $\sqrt{s}=7$ and $8$TeV via double parton scattering

Associated production of bottomonia and open charm hadrons in $pp$ collisions at $\sqrt{s}=7$ and $8$TeV is observed using data corresponding to an integrated luminosity of 3$fb^{-1}$ accumulated with the LHCb detector. The observation of five combinations, $\Upsilon(1S)D^0$, $\Upsilon(2S)D^0$, $\Upsilon(1S)D^+$, $\Upsilon(2S)D^+$ and $\Upsilon(1S)D^+_{s}$, is reported. Production cross-sections are measured for $\Upsilon(1S)D^0$ and $\Upsilon(1S)D^+$ pairs in the forward region. The measured cross-sections and the differential distributions indicate the dominance of double parton scattering as the main production mechanism. This allows a precise measurement of the effective cross-section for double parton scattering.

==> LHCb_HD_comma_separated_author_2015-08-11.tex <==
LHCb collaboration:
R. Aaij, 
C. Abell\'{a}n Beteta, 
B. Adeva, 
M. Adinolfi, 
A. Affolder, 
Z. Ajaltouni, 
S. Akar, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. An, 
L. Anderlini, 
J. Anderson, 
G. Andreassi, 
M. Andreotti, 
J.E. Andrews, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
P. d'Argent, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
A. Badalov, 
C. Baesso, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
V. Batozskaya, 
V. Battista, 
A. Bay, 
L. Beaucourt, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
L.J. Bel, 
V. Bellee, 
N. Belloli, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
A. Bertolin, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
P. Billoir, 
T. Bird, 
A. Birnkraut, 
A. Bizzeti, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
M. Borisyak, 
M. Borsato, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
S. Braun, 
M. Britsch, 
T. Britton, 
J. Brodzicka, 
N.H. Brook, 
E. Buchanan, 
C. Burr, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
R. Calabrese, 
M. Calvi, 
M. Calvo Gomez, 
P. Campana, 
D. Campora Perez, 
L. Capriotti, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
P. Carniti, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Cassina, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
G. Cavallero, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
M. Chefdeville, 
S. Chen, 
S.-F. Cheung, 
N. Chiapolini, 
M. Chrzaszcz, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
V. Cogoni, 
L. Cojocariu, 
G. Collazuol, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
M. Corvo, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
A. Crocombe, 
M. Cruz Torres, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
E. Dall'Occo, 
J. Dalseno, 
P.N.Y. David, 
A. Davis, 
O. De Aguiar Francisco, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
C.-T. Dean, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
M. Demmer, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
B. Dey, 
A. Di Canto, 
F. Di Ruscio, 
H. Dijkstra, 
S. Donleavy, 
F. Dordei, 
M. Dorigo, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
K. Dreimanis, 
L. Dufour, 
G. Dujany, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
S. Ely, 
S. Esen, 
H.M. Evans, 
T. Evans, 
A. Falabella, 
C. F\"{a}rber, 
N. Farley, 
S. Farry, 
R. Fay, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferrari, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
M. Fiorini, 
M. Firlej, 
C. Fitzpatrick, 
T. Fiutowski, 
K. Fohl, 
P. Fol, 
M. Fontana, 
F. Fontanelli, 
D. C. Forshaw, 
R. Forty, 
M. Frank, 
C. Frei, 
M. Frosini, 
J. Fu, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
S. Gallorini, 
S. Gambetta, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garc\'{i}a Pardi\~{n}as, 
J. Garra Tico, 
L. Garrido, 
D. Gascon, 
C. Gaspar, 
R. Gauld, 
L. Gavardi, 
G. Gazzoni, 
D. Gerick, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
S. Gian\`{i}, 
V. Gibson, 
O.G. Girard, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
E. Graverini, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
P. Griffith, 
L. Grillo, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
T. Hadavizadeh, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
X. Han, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
J. He, 
T. Head, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
L. Henry, 
E. van Herwijnen, 
M. He\ss, 
A. Hicheur, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
W. Hulsbergen, 
T. Humair, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
J. Jalocha, 
E. Jans, 
A. Jawahery, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
N. Jurik, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
S. Karodia, 
M. Kecke, 
M. Kelsey, 
I.R. Kenyon, 
M. Kenzie, 
T. Ketel, 
E. Khairullin, 
B. Khanji, 
C. Khurewathanakul, 
S. Klaver, 
K. Klimaszewski, 
O. Kochebina, 
M. Kolpin, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Kozeiha, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
W. Krzemien, 
W. Kucewicz, 
M. Kucharczyk, 
V. Kudryavtsev, 
A. K. Kuonen, 
K. Kurek, 
T. Kvaratskheliya, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
G. Lanfranchi, 
C. Langenbruch, 
B. Langhans, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
E. Lemos Cid, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
T. Likhomanenko, 
M. Liles, 
R. Lindner, 
C. Linn, 
F. Lionetto, 
B. Liu, 
X. Liu, 
D. Loh, 
I. Longstaff, 
J.H. Lopes, 
D. Lucchesi, 
M. Lucio Martinez, 
H. Luo, 
A. Lupato, 
E. Luppi, 
O. Lupton, 
A. Lusiani, 
F. Machefert, 
F. Maciuc, 
O. Maev, 
K. Maguire, 
S. Malde, 
A. Malinin, 
G. Manca, 
G. Mancinelli, 
P. Manning, 
A. Mapelli, 
J. Maratas, 
J.F. Marchand, 
U. Marconi, 
C. Marin Benito, 
P. Marino, 
J. Marks, 
G. Martellotti, 
M. Martin, 
M. Martinelli, 
D. Martinez Santos, 
F. Martinez Vidal, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
A. Mathad, 
Z. Mathe, 
C. Matteuzzi, 
A. Mauri, 
B. Maurin, 
A. Mazurov, 
M. McCann, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. Meadows, 
F. Meier, 
M. Meissner, 
D. Melnychuk, 
M. Merk, 
E Michielin, 
D.A. Milanes, 
M.-N. Minard, 
D.S. Mitzel, 
J. Molina Rodriguez, 
I.A. Monroy, 
S. Monteil, 
M. Morandin, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
J. Moron, 
A.B. Morris, 
R. Mountain, 
F. Muheim, 
D. M\"{u}ller, 
J. M\"{u}ller, 
K. M\"{u}ller, 
V. M\"{u}ller, 
M. Mussini, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
A. Nandi, 
I. Nasteva, 
M. Needham, 
N. Neri, 
S. Neubert, 
N. Neufeld, 
M. Neuner, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Novoselov, 
D.P. O'Hanlon, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
C.J.G. Onderwater, 
B. Osorio Rodrigues, 
J.M. Otalora Goicochea, 
A. Otto, 
P. Owen, 
A. Oyanguren, 
A. Palano, 
F. Palombo, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
L.L. Pappalardo, 
C. Pappenheimer, 
W. Parker, 
C. Parkes, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
C. Patrignani, 
A. Pearce, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
P. Perret, 
L. Pescatore, 
K. Petridis, 
A. Petrolini, 
M. Petruzzo, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
A. Pistone, 
A. Piucci, 
S. Playfer, 
M. Plo Casasus, 
T. Poikela, 
F. Polci, 
A. Poluektov, 
I. Polyakov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
E. Price, 
J.D. Price, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
R. Quagliani, 
B. Rachwal, 
J.H. Rademacker, 
M. Rama, 
M. Ramos Pernas, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
F. Redi, 
S. Reichert, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
S. Richards, 
M. Rihl, 
K. Rinnert, 
V. Rives Molina, 
P. Robbe, 
A.B. Rodrigues, 
E. Rodrigues, 
J.A. Rodriguez Lopez, 
P. Rodriguez Perez, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. W. Ronayne, 
M. Rotondo, 
T. Ruf, 
P. Ruiz Valls, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
V. Salustino Guimaraes, 
C. Sanchez Mayordomo, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
M. Santimaria, 
E. Santovetti, 
A. Sarti, 
C. Satriano, 
A. Satta, 
D.M. Saunders, 
D. Savrina, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
T. Schmelzer, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M. Schubiger, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
A. Semennikov, 
N. Serra, 
J. Serrano, 
L. Sestini, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
V. Shevchenko, 
A. Shires, 
B.G. Siddi, 
R. Silva Coutinho, 
L. Silva de Oliveira, 
G. Simi, 
M. Sirendi, 
N. Skidmore, 
T. Skwarnicki, 
E. Smith, 
E. Smith, 
I.T. Smith, 
J. Smith, 
M. Smith, 
H. Snoek, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
P. Spradlin, 
S. Sridharan, 
F. Stagni, 
M. Stahl, 
S. Stahl, 
S. Stefkova, 
O. Steinkamp, 
O. Stenyakin, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
S. Stracka, 
M. Straticiuc, 
U. Straumann, 
L. Sun, 
W. Sutcliffe, 
K. Swientek, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
T. Szumlak, 
S. T'Jampens, 
A. Tayduganov, 
T. Tekampe, 
M. Teklishyn, 
G. Tellarini, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
J. Todd, 
S. Tolk, 
L. Tomassetti, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
K. Trabelsi, 
M.T. Tran, 
M. Tresch, 
A. Trisovic, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
A. Ukleja, 
A. Ustyuzhanin, 
U. Uwer, 
C. Vacca, 
V. Vagnoni, 
G. Valenti, 
A. Vallier, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
M. Vieites Diaz, 
X. Vilasis-Cardona, 
V. Volkov, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
J.A. de Vries, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
J. Walsh, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
D. Websdale, 
A. Weiden, 
M. Whitehead, 
G. Wilkinson, 
M. Wilkinson, 
M. Williams, 
M.P. Williams, 
M. Williams, 
T. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
G. Wormser, 
S.A. Wotton, 
S. Wright, 
K. Wyllie, 
Y. Xie, 
Z. Xu, 
Z. Yang, 
J. Yu, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
L. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
S. Zucchelli

